Coronavirus Perceptions And Economic Anxiety

We provide one of the first systematic assessments of the development and determinants of economic anxiety at the onset of the coronavirus pandemic. Using a global dataset on internet searches and two representative surveys from the US, we document a substantial increase in economic anxiety during and after the arrival of the coronavirus. We also document a large dispersion in beliefs about the pandemic risk factors of the coronavirus, and demonstrate that these beliefs causally affect individuals' economic anxieties. Finally, we show that individuals' mental models of infectious disease spread understate non-linear growth and shape the extent of economic anxiety.

==> Final working paper/DiD_survey.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{2}{c}{Predicted impact on (standardized)}&\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{World}&\multicolumn{1}{c}{US}&\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
                &         &         &         &         \\
Any case        &0.2318\sym{**}&0.2579\sym{***}&0.2159\sym{*}&   0.0636\\
                & (0.0985)& (0.0946)& (0.1079)& (0.1258)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.07&     0.07&     0.08&     0.09\\
Number of Observations&     1920&     1920&     1920&     1920\\
\midrule Including controls&        X&        X&        X&        X\\
State FE        &        X&        X&        X&        X\\
Survey FE       &        X&        X&        X&        X\\
\bottomrule
\end{tabular}
}


==> Final working paper/Main_DD_results.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{4}{c}{Impact on Goolge search trends}\\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{Recession}&\multicolumn{1}{c}{Stock Market Crash}&\multicolumn{1}{c}{Conspiracy Theory}&\multicolumn{1}{c}{Survivalism}\\
\midrule
{\bf Panel  A: Any Covid-19 case}&         &         &         &         \\
                &         &         &         &         \\
Post any Covid-19 case&0.178\sym{**}&0.580\sym{***}&0.447\sym{***}&0.204\sym{***}\\
                &  (0.073)&  (0.124)&  (0.091)&  (0.073)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.04&     0.10&     0.06&     0.13\\
Number of Observations &    11640&    11640&    11640&    11640\\
\midrule {\bf Panel B: Any human-to-human transmission}&         &         &         &         \\
                &         &         &         &         \\
Post any human-to-human transmission&0.351\sym{**}&0.293\sym{*}&0.388\sym{**}&0.354\sym{**}\\
                &  (0.141)&  (0.163)&  (0.164)&  (0.140)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.04&     0.10&     0.06&     0.13\\
Number of Observations&    11640&    11640&    11640&    11640\\
 \midrule Number of countries&      194&      194&      194&      194\\
Country FE      &        X&        X&        X&        X\\
\bottomrule
\end{tabular}
}


==> Final working paper/Main_DD_results_nonormalization.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{4}{c}{Impact on Goolge search trends}\\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{Recession}&\multicolumn{1}{c}{Stock Market Crash}&\multicolumn{1}{c}{Conspiracy Theory}&\multicolumn{1}{c}{Survivalism}\\
\midrule
{\bf Panel  A: Any Covid-19 case}&         &         &         &         \\
                &         &         &         &         \\
Post any Covid-19 case&2.522\sym{***}&2.824\sym{***}&3.252\sym{***}&1.493\sym{***}\\
                &  (0.677)&  (0.538)&  (0.580)&  (0.443)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.27&     0.26&     0.31&     0.36\\
Number of Observations &    11640&    11640&    11640&    11640\\
\midrule {\bf Panel B: Any human-to-human transmission}&         &         &         &         \\
                &         &         &         &         \\
Post any human-to-human transmission&5.644\sym{***}&1.792\sym{*}&3.622\sym{*}&2.281\sym{**}\\
                &  (1.927)&  (1.069)&  (1.999)&  (0.978)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.27&     0.26&     0.31&     0.36\\
Number of Observations&    11640&    11640&    11640&    11640\\
 \midrule Number of countries&      194&      194&      194&      194\\
Country FE      &        X&        X&        X&        X\\
\bottomrule
\end{tabular}
}


==> Final working paper/Placebo_DD_results.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
\toprule
                &\multicolumn{10}{c}{Impact on google searches for}                                                 \\\cmidrule(lr){2-11}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
                &\multicolumn{1}{c}{Dog}&\multicolumn{1}{c}{Horse}&\multicolumn{1}{c}{Insect}&\multicolumn{1}{c}{DaVinci}&\multicolumn{1}{c}{Nelson Mandela}&\multicolumn{1}{c}{Rain}&\multicolumn{1}{c}{Rainbow}&\multicolumn{1}{c}{Stars}&\multicolumn{1}{c}{Mars (planet)}&\multicolumn{1}{c}{Menstrual Cycle}\\
\midrule
{\bf Panel  A: First confirmed case}&         &         &         &         &         &         &         &         &         &         \\
                &         &         &         &         &         &         &         &         &         &         \\
First confirmed case&   -0.018&   -0.036&   -0.007&   -0.044&   -0.033&    0.044&   -0.042&   -0.012&   -0.001&    0.033\\
                &  (0.018)&  (0.027)&  (0.042)&  (0.038)&  (0.058)&  (0.048)&  (0.045)&  (0.033)&  (0.103)&  (0.033)\\
                &         &         &         &         &         &         &         &         &         &         \\
\midrule R$^2$  &     0.05&     0.03&     0.02&     0.04&     0.03&     0.04&     0.03&     0.02&     0.06&     0.04\\
Number of Observations &    11640&    11640&    11639&    11249&    11483&    11640&    11640&    11640&    11507&    11477\\
\midrule {\bf Panel  B: First human-to-human  transmission}&         &         &         &         &         &         &         &         &         &         \\
                &         &         &         &         &         &         &         &         &         &         \\
First human-to-human  transmission&   -0.021&   -0.085&    0.035&   -0.030&    0.027&   -0.041&   -0.047&   -0.024&    0.102&    0.039\\
                &  (0.038)&  (0.064)&  (0.040)&  (0.039)&  (0.059)&  (0.078)&  (0.055)&  (0.048)&  (0.324)&  (0.028)\\
                &         &         &         &         &         &         &         &         &         &         \\
\midrule R$^2$  &     0.05&     0.03&     0.02&     0.04&     0.03&     0.04&     0.03&     0.02&     0.06&     0.04\\
Number of Observations&    11640&    11640&    11639&    11249&    11483&    11640&    11640&    11640&    11507&    11477\\
\midrule  Number of countries&      194&      194&      194&      193&      194&      194&      194&      194&      194&      193\\
Country FE      &        X&        X&        X&        X&        X&        X&        X&        X&        X&        X\\
Day FE          &        X&        X&        X&        X&        X&        X&        X&        X&        X&        X\\
\bottomrule
\end{tabular}
}


==> Final working paper/balance_experiment_main.tex <==
\begin{tabular}{l*{6}{c}} \toprule
          &\multicolumn{3}{c}{Mortality information experiment}&\multicolumn{3}{c}{Contagion information experiment}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{Mean low rel. mortality}&\multicolumn{1}{c}{Mean high rel. mortality}&\multicolumn{1}{c}{p(low rel. mort. = high rel. mort)}&\multicolumn{1}{c}{Mean no contagion info}&\multicolumn{1}{c}{Mean contagion info}&\multicolumn{1}{c}{p(no info = info)}\\
\midrule
\% Male   &    50.55&    47.49&     0.36&    50.11&    47.93&     0.51\\
\% Age < 35&    23.74&    24.62&     0.76&    23.96&    24.40&     0.88\\
\% Highschool education&    18.90&    16.34&     0.31&    16.70&    18.52&     0.47\\
\% College eductation&    78.90&    82.14&     0.22&    81.98&    79.08&     0.27\\
\% Currently working&    58.46&    51.63&     0.04&    55.38&    54.68&     0.83\\
\% Democrat&    38.90&    41.18&     0.48&    37.58&    42.48&     0.13\\
\% Republican&    33.41&    32.90&     0.87&    34.95&    31.37&     0.25\\
\% High trust in science&     1.98&     0.22&     0.01&     0.88&     1.31&     0.53\\
          &         &         &         &         &         &         \\
p-value of joint significance&         &         &     0.00&         &         &     0.74\\
\bottomrule \end{tabular}


==> Final working paper/comparison_time.tex <==
\begin{tabular}{l*{8}{c}} \toprule
          &\multicolumn{3}{c}{March 5}  &\multicolumn{3}{c}{March 16} &\multicolumn{2}{c}{Comparison of means}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
          &\multicolumn{1}{c}{Mean}&\multicolumn{1}{c}{SD}&\multicolumn{1}{c}{Obs.}&\multicolumn{1}{c}{Mean}&\multicolumn{1}{c}{SD}&\multicolumn{1}{c}{Obs.}&\multicolumn{1}{c}{$\Delta$}&\multicolumn{1}{c}{p(early = late)}\\
\midrule
\textbf{Panel A: Economic Anxieties}&         &         &         &         &         &         &         &         \\
          &         &         &         &         &         &         &         &         \\
\% agree: world severely affected by coronavirus&    80.12&    39.93&     1006&    67.61&    46.82&      914&   -12.50&    0.000\\
\% agree: US severely affected by coronavirus&    77.83&    41.56&     1006&    55.14&    49.76&      914&   -22.69&    0.000\\
\% worried about US economy&    87.57&    33.00&     1006&    68.05&    46.65&      914&   -19.52&    0.000\\
\% worried about personal econ. situation&    73.76&    44.02&     1006&    47.16&    49.95&      914&   -26.60&    0.000\\
          &         &         &         &         &         &         &         &         \\
\bottomrule \end{tabular}


==> Final working paper/contagion_cross_rand_check.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                &\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                &\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
{\bf Panel A: No control variables}&         &         \\
\midrule        &         &         \\
Contagion information&  -0.0107&-0.0876\sym{**}\\
                & (0.0435)& (0.0414)\\
                &         &         \\
\midrule R$^2$  &     0.57&     0.61\\
 Number of Observations &      914&      914\\
\midrule {\bf Panel B: Including control variables}&         &         \\
\midrule        &         &         \\
 Contagion information&  -0.0052&-0.0836\sym{**}\\
                & (0.0436)& (0.0415)\\
                &         &         \\
\midrule R$^2$  &     0.58&     0.62\\
 Number of Observations &      914&      914\\
\bottomrule
\end{tabular}
}


==> Final working paper/correlations_expgrowth_combined.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{8}{c}}
\toprule
                &\multicolumn{4}{c}{Predicted impact on (standardized)}&\multicolumn{4}{c}{Worry about (standardized)}\\\cmidrule(lr){2-5}\cmidrule(lr){6-9}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                &\multicolumn{1}{c}{World}&\multicolumn{1}{c}{World}&\multicolumn{1}{c}{US}&\multicolumn{1}{c}{US}&\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
                &         &         &         &         &         &         &         &         \\
{\bf Panel A }  &         &         &         &         &         &         &         &         \\
                &         &         &         &         &         &         &         &         \\
Log(estimate day 5)- z-score&0.0971\sym{***}&0.0832\sym{***}&0.0942\sym{***}&0.0893\sym{***}&0.0747\sym{**}&0.0750\sym{**}&   0.0044&   0.0268\\
                & (0.0284)& (0.0282)& (0.0299)& (0.0305)& (0.0306)& (0.0306)& (0.0318)& (0.0325)\\
                &         &         &         &         &         &         &         &         \\
\midrule R$^2$  &     0.01&     0.07&     0.01&     0.06&     0.01&     0.06&     0.00&     0.09\\
Number of Observations &     1006&     1006&     1006&     1006&     1006&     1006&     1006&     1006\\
\midrule        &         &         &         &         &         &         &         &         \\
{\bf Panel B}   &         &         &         &         &         &         &         &         \\
                &         &         &         &         &         &         &         &         \\
Log(estimate day 10)- z-score&0.1044\sym{***}&0.0857\sym{***}&0.1137\sym{***}&0.1069\sym{***}&0.0714\sym{**}&0.0703\sym{**}&  -0.0229&   0.0086\\
                & (0.0291)& (0.0292)& (0.0295)& (0.0303)& (0.0313)& (0.0314)& (0.0327)& (0.0321)\\
                &         &         &         &         &         &         &         &         \\
\midrule R$^2$  &     0.01&     0.07&     0.01&     0.06&     0.01&     0.06&     0.00&     0.09\\
Number of Observations &     1006&     1006&     1006&     1006&     1006&     1006&     1006&     1006\\
\midrule        &         &         &         &         &         &         &         &         \\
{\bf Panel C}   &         &         &         &         &         &         &         &         \\
                &         &         &         &         &         &         &         &         \\
Log(estimate day 20)- z-score&0.0828\sym{***}&0.0608\sym{*}&0.0933\sym{***}&0.0841\sym{***}&   0.0502&   0.0489&  -0.0441&  -0.0079\\
                & (0.0313)& (0.0315)& (0.0314)& (0.0323)& (0.0324)& (0.0326)& (0.0332)& (0.0327)\\
                &         &         &         &         &         &         &         &         \\
\midrule R$^2$  &     0.01&     0.06&     0.01&     0.06&     0.00&     0.06&     0.00&     0.09\\
Number of Observations &     1006&     1006&     1006&     1006&     1006&     1006&     1006&     1006\\
\midrule Controls&         &        X&         &        X&         &        X&         &        X\\
\bottomrule
\end{tabular}
}


==> Final working paper/eiu-recession_hits-leadingindicator.tex <==
L.Recession topic Google searches&      -1.009***&      -1.231*  &      -1.564***&      -1.847   &      -1.345   &       1.109*  &      -5.063***\\
                    &     (0.311)   &     (0.661)   &     (0.506)   &     (1.798)   &     (0.888)   &     (0.657)   &     (1.352)   \\
                    &               &               &               &               &               &               &               \\
R$^2$               &        .716   &        .446   &        .627   &         .27   &        .282   &        .236   &        .314   \\
Countries           &          70   &          72   &          58   &          58   &          58   &          58   &          58   \\
Observations        &        1350   &        1218   &        1087   &        1087   &        1087   &        1087   &        1087   \\


==> Final working paper/experiment_correlations_combined.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{2}{c}{Predicted impact on (standardized)}&\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{World}&\multicolumn{1}{c}{US}&\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
{\bf Panel A: No control variables}&         &         &         &         \\
                &         &         &         &         \\
Overestimate mortality&0.3655\sym{***}&0.4516\sym{***}&0.1892\sym{***}&0.4783\sym{***}\\
                & (0.0647)& (0.0637)& (0.0655)& (0.0635)\\
                &         &         &         &         \\
Overestimate contagiousness&0.5263\sym{***}&0.5722\sym{***}&0.4504\sym{***}&0.4096\sym{***}\\
                & (0.0899)& (0.0843)& (0.0879)& (0.0825)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.08&     0.11&     0.04&     0.09\\
\midrule        &         &         &         &         \\
                &         &         &         &         \\
{\bf Panel B: Including control variables}&         &         &         &         \\
                &         &         &         &         \\
Overestimate mortality&0.3830\sym{***}&0.4390\sym{***}&0.1850\sym{***}&0.4016\sym{***}\\
                & (0.0654)& (0.0642)& (0.0668)& (0.0645)\\
                &         &         &         &         \\
Overestimate contagiousness&0.5077\sym{***}&0.5392\sym{***}&0.4252\sym{***}&0.3780\sym{***}\\
                & (0.0885)& (0.0832)& (0.0849)& (0.0810)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.13&     0.16&     0.10&     0.16\\
 Number of Observations &      914&      914&      914&      914\\
\bottomrule
\end{tabular}
}


==> Final working paper/experiment_correlations_combined_continuous.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{2}{c}{Predicted impact on (standardized)}&\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{World}&\multicolumn{1}{c}{US}&\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
{\bf Panel A: No control variables}&         &         &         &         \\
                &         &         &         &         \\
Perceived mortality&0.8220\sym{***}&1.1333\sym{***}&0.6213\sym{***}&1.3450\sym{***}\\
                & (0.1887)& (0.1730)& (0.2013)& (0.1841)\\
                &         &         &         &         \\
Perceived contagiousness &0.2714\sym{**}&0.6121\sym{***}&0.4826\sym{***}&0.5845\sym{***}\\
                & (0.1243)& (0.1071)& (0.1200)& (0.1149)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.03&     0.09&     0.04&     0.11\\
\midrule        &         &         &         &         \\
                &         &         &         &         \\
{\bf Panel B: Including control variables}&         &         &         &         \\
                &         &         &         &         \\
Perceived mortality&0.8841\sym{***}&1.1090\sym{***}&0.6747\sym{***}&1.1382\sym{***}\\
                & (0.1932)& (0.1804)& (0.2098)& (0.1919)\\
                &         &         &         &         \\
Perceived contagiousness&0.2728\sym{**}&0.6084\sym{***}&0.4810\sym{***}&0.5596\sym{***}\\
                & (0.1239)& (0.1070)& (0.1226)& (0.1187)\\
                &         &         &         &         \\
\midrule R$^2$  &     0.08&     0.14&     0.10&     0.17\\
 Number of Observations &      914&      914&      914&      914\\
\bottomrule
\end{tabular}
}


==> Final working paper/experiment_mainpart1_combined.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                &\multicolumn{2}{c}{Predicted impact on (standardized)}\\\cmidrule(lr){2-3}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                &\multicolumn{1}{c}{World}&\multicolumn{1}{c}{US}\\
\midrule
{\bf Panel A: No control variables} &         &         \\
                &         &         \\
High relative mortality&0.2833\sym{***}&0.2246\sym{***}\\
                & (0.0655)& (0.0658)\\
                &         &         \\
\midrule R$^2$  &     0.02&     0.01\\
 Number of Observations &      914&      914\\
\midrule        &         &         \\
                &         &         \\
{\bf Panel B: Including control variables} &         &         \\
                &         &         \\
High relative mortality&0.2705\sym{***}&0.2245\sym{***}\\
                & (0.0659)& (0.0651)\\
                &         &         \\
\midrule R$^2$  &     0.06&     0.07\\
 Number of Observations &      914&      914\\
\bottomrule
\end{tabular}
}


==> Final working paper/experiment_mainpart2_combined.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                &\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                &\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
{\bf Panel A: No control variables}&         &         \\
                &         &         \\
High relative mortality&0.1557\sym{**}&0.1560\sym{**}\\
                & (0.0660)& (0.0660)\\
                &         &         \\
\midrule R$^2$  &     0.01&     0.01\\
 Number of Observations &      914&      914\\
\midrule        &         &         \\
Contagion information&  -0.0116&-0.0866\sym{**}\\
                & (0.0434)& (0.0415)\\
                &         &         \\
\midrule R$^2$  &     0.57&     0.61\\
 Number of Observations &      914&      914\\
\midrule        &         &         \\
{\bf Panel B: Including control variables}&         &         \\
                &         &         \\
High relative mortality&0.1556\sym{**}&0.1834\sym{***}\\
                & (0.0660)& (0.0645)\\
                &         &         \\
\midrule R$^2$  &     0.07&     0.10\\
 Number of Observations &      914&      914\\
\midrule        &         &         \\
Contagion information&  -0.0064&-0.0826\sym{**}\\
                & (0.0435)& (0.0416)\\
                &         &         \\
\midrule R$^2$  &     0.58&     0.62\\
 Number of Observations &      914&      914\\
\bottomrule
\end{tabular}
}


==> Final working paper/growth_perc_pred.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                &\multicolumn{2}{c}{Log predicted cases after twenty days}&\multicolumn{2}{c}{Exponential mental model}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{Post LASSO }&\multicolumn{1}{c}{OLS}&\multicolumn{1}{c}{Post LASSO }\\
\midrule
Male            &    0.236         &    0.213         &   0.0163         &                  \\
                &  (0.287)         &  (0.285)         & (0.0240)         &                  \\
Aged 25 to 34   &  -0.0312         &   -0.244         & 0.000318         &  -0.0361         \\
                &  (0.490)         &  (0.381)         & (0.0415)         & (0.0300)         \\
Aged 35 to 44   &    0.153         &   -0.115         &   0.0539         &                  \\
                &  (0.531)         &  (0.407)         & (0.0455)         &                  \\
Aged 45 to 54   &    0.296         &                  &  -0.0193         &  -0.0603\sym{**} \\
                &  (0.495)         &                  & (0.0398)         & (0.0272)         \\
Aged 55 to 64   &    0.536         &    0.354         &   0.0400         &                  \\
                &  (0.534)         &  (0.421)         & (0.0431)         &                  \\
Aged 65 above   &    1.289\sym{**} &    1.097\sym{**} &    0.138\sym{***}&    0.106\sym{***}\\
                &  (0.560)         &  (0.450)         & (0.0472)         & (0.0353)         \\
Log income      &    2.792         &    0.370\sym{**} &    0.387         &   0.0342\sym{**} \\
                &  (3.450)         &  (0.182)         &  (0.271)         & (0.0139)         \\
Log income squared&   -0.113         &                  &  -0.0166         &                  \\
                &  (0.162)         &                  & (0.0127)         &                  \\
Highschool education&    1.265\sym{**} &                  &   0.0793\sym{**} &                  \\
                &  (0.499)         &                  & (0.0370)         &                  \\
College eductation&    2.257\sym{***}&    1.184\sym{***}&    0.144\sym{***}&   0.0781\sym{***}\\
                &  (0.477)         &  (0.314)         & (0.0354)         & (0.0255)         \\
Currently working&   -0.687\sym{*}  &   -0.667\sym{*}  &  -0.0428         &  -0.0366         \\
                &  (0.379)         &  (0.373)         & (0.0322)         & (0.0278)         \\
Student         &   -0.804         &   -0.780         &  -0.0317         &                  \\
                &  (0.602)         &  (0.601)         & (0.0472)         &                  \\
Democrat        &   -0.658\sym{**} &   -0.642\sym{*}  &  -0.0420         &  -0.0346         \\
                &  (0.330)         &  (0.329)         & (0.0278)         & (0.0230)         \\
Republican      &   -0.359         &   -0.336         &  -0.0165         &                  \\
                &  (0.376)         &  (0.376)         & (0.0302)         &                  \\
Constant        &   -12.79         &    1.335         &   -2.215         &   -0.250\sym{*}  \\
                &  (18.34)         &  (1.764)         &  (1.436)         &  (0.140)         \\
\midrule
R$^2$           &   0.0517         &   0.0485         &   0.0559         &   0.0510         \\
Number of observations&     1006         &     1006         &     1006         &     1006         \\
\bottomrule
\end{tabular}
}


==> Final working paper/sum_expgrowth.tex <==
\begin{tabular}{l*{4}{c}} \toprule
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
          &\multicolumn{1}{c}{Mean}&\multicolumn{1}{c}{SD}&\multicolumn{1}{c}{Median}&\multicolumn{1}{c}{Obs.}\\
\midrule
\textbf{Panel A: Demographics}&         &         &         &         \\
          &         &         &         &         \\
\%  Male  &    52.09&    49.98&         &     1006\\
\%  Age < 35&    22.66&    41.89&         &     1006\\
\% Highschool education&    19.98&    40.00&         &     1006\\
\%  College eductation&    76.64&    42.33&         &     1006\\
\% Currently working&    52.19&    49.98&         &     1006\\
\% Democrat&    38.57&    48.70&         &     1006\\
\%  Republican&    32.11&    46.71&         &     1006\\
\% High trust in science&     1.79&    13.26&         &     1006\\
          &         &         &         &         \\
\textbf{Panel B: Economic Anxieties}&         &         &         &         \\
          &         &         &         &         \\
\% agree: world severely affected by coronavirus&    80.12&    39.93&         &     1006\\
\% agree: US severely affected by coronavirus&    77.83&    41.56&         &     1006\\
\% worried about US economy&    87.57&    33.00&         &     1006\\
\% worried about personal econ. situation&    73.76&    44.02&         &     1006\\
          &         &         &         &         \\
\textbf{Panel C: Coronavirus perceptions }&         &         &         &         \\
          &         &         &         &         \\
Infectiousness (R0)&    49.81&   175.13&        5&     1006\\
Number of cases after 5 days (w)&    20.02&    20.72&       11&     1006\\
Number of cases after 10 days  (w)&   340.29&   678.64&       30&     1006\\
Number of cases after 20 days  (w)&122218.17&311256.66&       60&     1006\\
Predicted  mortality rate&    15.60&    21.47&        5&     1006\\
\bottomrule \end{tabular}


==> Final working paper/sumstats_experiment_main.tex <==
\begin{tabular}{l*{4}{c}} \toprule
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
          &\multicolumn{1}{c}{Mean}&\multicolumn{1}{c}{SD}&\multicolumn{1}{c}{Median}&\multicolumn{1}{c}{Obs.}\\
\midrule
\textbf{Panel A: Demographics}&         &         &         &         \\
          &         &         &         &         \\
\%  Male  &    49.02&    50.02&         &      914\\
\%  Age < 35&     0.23&     0.42&         &      914\\
\% Highschool education&    17.61&    38.12&         &      914\\
\%  College eductation&    80.53&    39.62&         &      914\\
\% Currently working&    55.03&    49.77&         &      914\\
\% Democrat&    40.04&    49.03&         &      914\\
\%  Republican&    33.15&    47.10&         &      914\\
\% High trust in science&     1.09&    10.41&         &      914\\
          &         &         &         &         \\
\textbf{Panel B: Economic Anxieties}&         &         &         &         \\
          &         &         &         &         \\
\% agree: world severely affected by coronavirus&    67.61&    46.82&         &      914\\
\% agree: US severely affected by coronavirus&    55.14&    49.76&         &      914\\
\% worried about US economy&    68.05&    46.65&         &      914\\
\% worried about personal econ. situation&    47.16&    49.95&         &      914\\
          &         &         &         &         \\
\textbf{Panel C: Coronavirus perceptions }&         &         &         &         \\
          &         &         &         &         \\
Infectiousness (R0)&    43.23&   146.17&       10&      914\\
Predicted  mortality rate&    13.70&    20.84&        5&      914\\
\bottomrule \end{tabular}


==> Final working paper/table-roper-poll-anycovid_confirmed.tex <==
Any Covid-19 case   &       0.111*  &       0.124** &       0.123** \\
                    &     (0.063)   &     (0.057)   &     (0.056)   \\
                    &               &               &               \\
Mean of DV          &      .00278   &      .00213   &     .000396   \\
R$^2$               &        .179   &        .139   &        .186   \\
States              &          50   &          50   &          50   \\
Observations        &        1197   &        1192   &        1197   \\


==> Final working paper/treatment_interaction_effects.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                &\multicolumn{2}{c}{Worry about (standardized)}\\\cmidrule(lr){2-3}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                &\multicolumn{1}{c}{US Economy}&\multicolumn{1}{c}{Pers. Economic Sit.}\\
\midrule
{\bf Panel A: No control variables}&         &         \\
\midrule        &         &         \\
Contagion information&   0.0270&-0.1243\sym{**}\\
                & (0.0576)& (0.0493)\\
                &         &         \\
Contagion information $\times$ Low relative mortality&  -0.0759&   0.0743\\
                & (0.0675)& (0.0571)\\
                &         &         \\
Baseline value  &0.7534\sym{***}&0.7803\sym{***}\\
                & (0.0248)& (0.0228)\\
                &         &         \\
\midrule R$^2$  &     0.57&     0.61\\
 Number of Observations &      914&      914\\
\midrule {\bf Panel B: Including control variables}&         &         \\
\midrule        &         &         \\
Contagion information&   0.0427&-0.1188\sym{**}\\
                & (0.0576)& (0.0494)\\
                &         &         \\
  Contagion information $\times$ Low relative mortality&  -0.0965&   0.0709\\
                & (0.0667)& (0.0567)\\
                &         &         \\
Baseline value  &0.7467\sym{***}&0.7572\sym{***}\\
                & (0.0259)& (0.0250)\\
                &         &         \\
\midrule R$^2$  &     0.58&     0.62\\
 Number of Observations &      914&      914\\
\bottomrule
\end{tabular}
}

